On the Use of Context for Predicting Citation Worthiness of Sentences in Scholarly Articles

In this paper, we study the importance of context in predicting the citation worthiness of sentences in scholarly articles. We formulate this problem as a sequence labeling task solved using a hierarchical BiLSTM model. We contribute a new benchmark dataset containing over two million sentences and their corresponding labels. We preserve the sentence order in this dataset and perform document-level train/test splits, which importantly allows incorporating contextual information in the modeling process. We evaluate the proposed approach on three benchmark datasets. Our results quantify the benefits of using context and contextual embeddings for citation worthiness. Lastly, through error analysis, we provide insights into cases where context plays an essential role in predicting citation worthiness.

==> discussion.tex <==



==> figure.tex <==
\begin{comment}
\begin{figure}
\centering
\begin{tikzpicture}
\node[text height=0.3cm] (y1) {$l_1$};
\node[text height=0.3cm] (y2) [right=of y1] {$l_2$};
\node[text height=0.3cm] (y3) [right=of y2] {$l_3$};
\node[text height=0.3cm] (yn) [right=of y3] {$l_n$};
\node[box,fill=black!10] (h1) [below=0.5 of y1] {$\overleftrightarrow{h_1}$};
\node[box,fill=black!10] (h2) [below=0.5 of y2] {$\overleftrightarrow{h_2}$};
\node[box,fill=black!10] (h3) [below=0.5 of y3] {$\overleftrightarrow{h_3}$};
\node[box,fill=black!10] (hn) [below=0.5 of yn] {$\overleftrightarrow{h_n}$};
\node[text height=0.3cm] (x1) [below=0.5 of h1] {$x_1$};
\node[text height=0.3cm] (x2) [below=0.5 of h2] {$x_2$};
\node[text height=0.3cm] (x3) [below=0.5 of h3] {$x_3$};
\node[text height=0.3cm] (xn) [below=0.5 of hn] {$x_n$};
\node[text height=0.3cm] (bert1) [below=0.5 of x1] {};
\node[text height=0.3cm] (bert2) [below=0.5 of x2] {};
\node[text height=0.3cm] (bert3) [below=0.5 of x3] {};
\node[text height=0.3cm] (bertn) [below=0.5 of xn] {};
\node[text height=0.3cm] (s1) [below=0.5 of bert1] {$s_1$};
\node[text height=0.3cm] (s2) [below=0.5 of bert2] {$s_2$};
\node[text height=0.3cm] (s3) [below=0.5 of bert3] {$s_3$};
\node[text height=0.3cm] (sn) [below=0.5 of bertn] {$s_n$};
\node[text width=2cm] (BiLSTM) [right=0.5cm of hn] {BiLSTM};
\node[text width=2cm] (Input) [right=0.5 of sn] {Sentences};
\node[text width=2cm] (Output) [right=0.5 of yn] {Outputs};
\node[text width=2cm] (BertLayer) [right=0.5 of bertn] {Embedding Layer};
\node[text width=2cm] (Embeddings) [right=0.5 of xn] {Embeddings};
\node[box,minimum width=5.5cm] (bert) [left=0.2 of BertLayer] {Contextual Embedding};
\path (y3) -- node[auto=false]{\ldots} (yn);
\draw[latex'-latex'] (h1) -- node[] {} (h2);
\draw[latex'-latex'] (h2) -- node[] {} (h3);
\path (h3) -- node[auto=false] {\ldots} (hn);
\path (h1) edge [connect] (y1);
\path (h2) edge [connect] (y2);
\path (h3) edge [connect] (y3);
\path (hn) edge [connect] (yn);
\path (x1) edge [connect] (h1);
\path (x2) edge [connect] (h2);
\path (x3) edge [connect] (h3);
\path (xn) edge [connect] (hn);
\path (bert1) edge [connect] (x1);
\path (bert2) edge [connect] (x2);
\path (bert3) edge [connect] (x3);
\path (bertn) edge [connect] (xn);
\path (s1) edge [connect] (bert1);
\path (s2) edge [connect] (bert2);
\path (s3) edge [connect] (bert3);
\path (sn) edge [connect] (bertn);
\path (s3) -- node[auto=false]{\ldots} (sn);
\end{tikzpicture}
\caption{BiLSTM architecture for citation worthiness.}
\label{fig:architecture}
\end{figure}
\end{comment}

==> related.tex <==
Citation worthiness is very closely related to citation recommendation, where the goal is to recommend a reference for a sentence in a scientific article. Many of these studies have proposed techniques that incorporate local context into the ranking process. \cite{strohman2007recommending} linearly combine text and citation-based features to generate scores for the final ranking task. \cite{he2010context} designed a context-aware non-parametric probabilistic model to measure the relevance between a citation and a document. More recently, neural networks have been explored by \cite{huang2015neural, ebesu2017neural} to select and rank citations for a given article. \cite{cai2018three, yang2018lstm, cai2018generative} further extended the research area by combining penalization into the recommendation process.  

Citation analysis, another closely related research domain, aims to predict the sentiment and purpose of a citation. \cite{athar2012context} used the context to predict the sentiment of a citation and explored the effects of context size on the final performance. \cite{abu2013purpose} presented a sequence labeling model that identifies the context and classifies the polarity. \cite{athar2011sentiment} explored the effectiveness of structured-based features for this task. While most of the current research trains separate models for the sentiment and purpose identification tasks, \cite{yousif2019multi} proposed a multi-task learning setup that jointly learns the objectives for these two tasks. 

Recognizing and understanding the author's motivation behind a citation has also been well studied by NLP researchers, commonly referred to as citation function classification. \cite{teufel2006automatic} proposed a new annotation scheme and explored supervised learning to solve this task. \cite{li2013towards} expanded on this annotation scheme by including more functions and implementing a Maximum Entropy-based system to classify citation functions automatically. Recently, \cite{hernandez2017citation} presented a new annotation scheme that produces a more granular set of categories for this classification task.

% Citations within the scientific literature have been well studied in the context of problems that are closely related to the task of citation worthiness. One such research area involves applying machine learning models towards the goal of recommending citations for a given scientific article. Many of these studies have proposed techniques that incorporate local context into the ranking process.
% \cite{strohman2007recommending} linearly combines text and citation based features in order to generate scores for the final ranking task. \cite{he2010context} designed a context-aware non-parametric probabilistic model to measure the relevance between a citation and a document. Very recently neural networks have been explored by \cite{huang2015neural, ebesu2017neural} to select and rank citations for a given article. \cite{cai2018three, yang2018lstm, cai2018generative} further extended the research area by combining penalization into the recommendation process.  

% Citation Analysis is a research area that studies and predicts the sentiment and purpose of a citation with respect to the citation context. \cite{athar2012context} applies the context towards predicting the sentiment of a citation and explores the effects of context size on the final performance. \cite{abu2013purpose} presented a sequence labeling model that identifies the context and classifies polarity based on it. \cite{athar2011sentiment} explores in detail the effectiveness of structured based features for this task. While most of the current research trains separate models for the sentiment and purpose identification tasks, \cite{yousif2019multi} proposed a multi-task learning setup that jointly learns the objectives for these two tasks. 

% Recognizing and understanding the author's motivation behind a citation has also been well studied by researchers from different fields. This task is commonly referred as citation function classification. \cite{teufel2006automatic} proposed a new annotation scheme and further explored supervised learning to solve the task. Later \cite{li2013towards} expanded on this annotation scheme by including more functions and implemented a Maximum Entropy-based system to automatically classify citation functions. Recently \cite{hernandez2017citation} presented a new annotation scheme that manages to produce more granular set of categories for the classification task.
